Modular and Incremental Global Model Management with Extended Generalized Discrimination Networks

Complex projects developed under the paradigm of model-driven engineering nowadays often involve several interrelated models, which are automatically processed via a multitude of model operations. Modular and incremental construction and execution of such networks of models and model operations are required to accommodate efficient development with potentially large-scale models. The underlying problem is also called Global Model Management. In this report, we propose an approach to modular and incremental Global Model Management via an extension to the existing technique of Generalized Discrimination Networks (GDNs). In addition to further generalizing the notion of query operations employed in GDNs, we adapt the previously query-only mechanism to operations with side effects to integrate model transformation and model synchronization. We provide incremental algorithms for the execution of the resulting extended Generalized Discrimination Networks (eGDNs), as well as a prototypical implementation for a number of example eGDN operations. Based on this prototypical implementation, we experiment with an application scenario from the software development domain to empirically evaluate our approach with respect to scalability and conceptually demonstrate its applicability in a typical scenario. Initial results confirm that the presented approach can indeed be employed to realize efficient Global Model Management in the considered scenario.

==> sections/3_related_work.tex <==
% !TeX root = ../tr_migmm_properties.tex

\section{Related Work (Global Model Management)}\label{sec:related_work}

There already exists a significant body of research that aims to tackle the problem of modular and incremental construction and execution of networks of model operations from different directions.

\textbf{Global Model Management:} Global Model Management, also called modeling in the large \cite{bezivin2004modeling}, employs so-called mega models \cite{bezivin2004need} to explicitly represent models and related model operations to facilitate dedicated management of such networks of models and model operations. However, current solutions only offer limited support for modular composition of model operations or incremental execution or employ a restricted notion of model operations.

In \cite{stevens2017bidirectional}, a technique for Global Model Management is presented based on bidirectional model synchronizations. The solution in \cite{stevens2017bidirectional} requires all model operations to be bidirectional synchronizations and hence does not provide dedicated support for modular construction and execution of query operations such as model properties. Furthermore, \cite{stevens2017bidirectional} also only provides an execution algorithm for model operation networks with a restricted structure for which termination with a correct result can be formally guaranteed, but which networks used in practice may not always adhere to. In \cite{stevens2020connecting}, the approach is extended with a so-called orientation model, which steers network execution and thereby relaxes the structural restrictions.

A comprehensive approach to Global Model Management is presented in \cite{seibel2010dynamic} in the form of dynamic hierarchic megamodels. While the solution in \cite{seibel2010dynamic} supports incremental execution of various model operations, it has only limited support for modularity by requiring an implicit export of model elements into a global context to facilitate the interplay between operations. Moreover, modular construction of model operations in the form of queries from suboperations and in particular the important RETE mechanism is not natively supported.

==> sections/7_related_work_2.tex <==
% !TeX root = ../tr_migmm_properties.tex

\section{Related Work}

\textbf{Discrimination Networks:} Another direction are discrimination networks as discussed in Section \ref{sec:discrimination_networks}. By representing model queries as networks of subqueries with well-defined interfaces in the form of indexers or marking model elements, discrimination networks enable modular construction of certain networks of model operations via composition, as well as incremental execution. However, discrimination networks are usually primarily employed for model querying and only have limited or no capabilities for the integration of model operations with side-effects.

The perhaps most notable realization of discrimination networks in the context of model-driven engineering is the VIATRA framework \cite{varro2016}, which allows the specification of model queries in the VQL language. Notably, VQL supports the composition of queries from subqueries. VIATRA's incremental execution engine is based on RETE nets with their restricted structure. In addition to executing model queries, the engine is also able to perform model transformation and synchronization operations in reaction to updates to a query's results. However, while VQL provides a multitude of advanced constructs for specifying model queries including negative patterns, attribute conditions and aggregation, VIATRA does not consider seamless integration of model operations specified in other languages or executed by different engines. This limits possible queries to what can be expressed in VQL and also means that VIATRA only supports a certain notion of reactive model transformation and synchronization. Other mechanisms such as triple graph grammars are not supported within the framework. Finally, VIATRA is not intended as a framework for modeling in the large, meaning that the overall network of model operations remains implicit.

Generalized Discrimination Networks were originally in the context of relational database management systems \cite{hanson2002trigger}. The work in \cite{hanson2002trigger} hence lacks an explicit connection to model-driven engineering. Thus, it also exclusively considers operations in the form of queries, that is, it does not provide any support for operations with side-effects.

Similarly, the realization by Beyhl et al. in the context of model-driven engineering \cite{beyhl2016operationalization} focuses solely on the execution of queries. While the approach in \cite{beyhl2016operationalization} supports a fairly expressive notion of queries in the form of nested graph conditions and provides a clear notion of modularity and incrementality via its definition of GDN nodes along with an incremental algorithm for GDN execution, certain query-related operations such as aggregation are not supported by the underlying formalism. Moreover, while GDN nodes are implemented via in-place model transformations, these transformations are limited to creating and deleting markings and may not modify the actual models.

\textbf{Model View Approaches:} Another related field of research are model view approaches \cite{bruneliere2019feature}, which investigate the problem of managing multiple views on a system that may be specified via a collection of interlinked models. Keeping these views consistent requires the orchestrated execution of networks of consistency preserving operations. Existing solutions however often restrict the structure of the network of model operations or consider only certain kinds of operations. Furthermore, due to their different focus in contrast to discrimination networks, model view approaches do not explicitly consider the modular composition of model operations from suboperations required for complex model properties and usually do not consider intra-model consistency constraints or.

Some model view approaches are based on the notion of a single underlying model (SUM) from which the individual views (which can be seen as queries or models in their own right) are derived \cite{atkinson2009orthographic}, which effectively introduces substantial restrictions on the structure of the network of operations.

The Vitruvius approach \cite{klare2021enabling} employs a so-called virtual single underlying model, which does not actually materialize an integration of the different system models. While Vitruvius has a dedicated incremental algorithm for executing complex networks of consistency preservation operations, its notion of consistency is limited to relations between pairs of tuples of model elements, which does not support operations such as aggregation. Vitruvius also deliberately does not consider intra-model consistency or composition of model properties.
